Self-Assessment for Single-Object Tracking in Clutter Using Subjective Logic

Reliable tracking algorithms are essential for automated driving. However, the existing consistency measures are not sufficient to meet the increasing safety demands in the automotive sector. Therefore, this work presents a novel method for self-assessment of single-object tracking in clutter based on Kalman filtering and subjective logic. A key feature of the approach is that it additionally provides a measure of the collected statistical evidence in its online reliability scores. In this way, various aspects of reliability, such as the correctness of the assumed measurement noise, detection probability, and clutter rate, can be monitored in addition to the overall assessment based on the available evidence. Here, we present a mathematical derivation of the reference distribution used in our self-assessment module for our studied problem. Moreover, we introduce a formula that describes how a threshold should be chosen for the degree of conflict, the subjective logic comparison measure used for the reliability decision making. Our approach is evaluated in a challenging simulation scenario designed to model adverse weather conditions. The simulations show that our method can significantly improve the reliability checking of single-object tracking in clutter in several aspects.

==> resources/figures/BiOpinion.tex <==
%\documentclass[tikz, border=2pt]{standalone}

%Pakete einbinden
%\usepackage[T1]{fontenc}        % Aktiviert EC-Schriftarten
%\usepackage[utf8]{inputenc}     % Dateikodierung
%\usepackage{lmodern}            % Latin Modern
%\usepackage[ngerman]{babel}     % Deutsche Einstellungen
%\usepackage{siunitx}            % SI Einheiten und Zahlenformatierung
%\usepackage{upgreek}            % Aufrechte griechische Buchstaben im Mathemodus
%\usepackage{amsmath}            % bessere Mathematik
%\usepackage{xcolor}
%\usepackage{tikz}
%\usepackage{pgfplots}
%\pgfplotsset{compat=newest}
%\usepackage{varwidth}

%\usetikzlibrary{plotmarks}
%\usepgfplotslibrary{patchplots}
%\usetikzlibrary{math}
%\usetikzlibrary{calc}
%\usetikzlibrary{intersections}




%\begin{document}
\begin{tikzpicture}[scale=1.5, line join = round, line cap = round]

\footnotesize
%\newlength\breite
%\setlength\breite{\textwidth}
\definecolor{grey}{HTML}{D3D3D3}

        % set up some factors and lengths
        \tikzmath{\a = 2; \h=\a*sqrt(3)/2; \dy=\a/2/sqrt(3);}
        
        % set up coordinates
        \coordinate (O) at (0,0);
        \coordinate (Xn) at (-\a/2,-\dy);
        \path (Xn) ++(\a,0) coordinate (X);
        \path (X) ++(120:\a) coordinate (U);
        \path (Xn) ++(30:\h*0.8) coordinate (w);
        \path (Xn) -- ($(Xn)!0.85!(X)$) coordinate (a);
        \path[name path=linie1] (Xn) -- (X);
        \path[name path=linie2] (Xn) -- (U);
        \path[name path=linie3] (U) -- (X);
        
        \draw[line width=1pt] (Xn) -- (X) -- (U) --cycle;
        
        % labels
        \node[anchor=east, align=center, fill=white, inner sep=0pt, outer sep=1pt] at (Xn) {$\bar{x}$};
        \node[anchor=west, align=center, fill=white, inner sep=0pt, outer sep=1pt] at (X) {$x$};
        \node[anchor=south, align=center, fill=white, inner sep=0pt, outer sep=1pt] at (U) {$u$};
        \fill[black] (a) circle (0.4pt) node[anchor=north,xshift=+0.1cm] at (a) {$a_x$};
        \node[anchor=north east] at (w) {$\omega_X$};
        
        % director
        \draw[dashed] (U) -- node[pos=0.8, above, sloped, inner sep=0pt, outer sep=1pt] {\scriptsize{director}} (a);
        
        % calculate P
        \path (U) -- ($(U)!0.6!(a)$) coordinate (h);
        \path[name path=proj] (w) -- +($(a)-(h)$);
        \path[name intersections={of=linie1 and proj,by=E}];
        \fill[black] (E) circle (0.4pt);
        \draw[dashed] (w) --node[pos=0.5, above, sloped, inner sep=0pt, outer sep=1pt] {\scriptsize{projector}} (E);
        \fill[black] (E) circle (0.4pt) node[anchor=north, xshift=-0.1cm] at (E) {$P(x)$};
        
        % lines
        \path[name path=linieB] (w) -- ++(150:0.35*\a);
        \path[name intersections={of=linie2 and linieB,by=B}];
        \path[name path=linieD] (w) -- ++(30:0.2*\a);
        \path[name intersections={of=linie3 and linieD,by=D}];
        \path[name path=linieU] (w) -- ++(-90:0.35*\a);
        \path[name intersections={of=linie1 and linieU,by=Un}];
        
        % Linien für b, d, u
        \draw (w) --node[inner sep=0pt, fill=white, outer sep=1pt] {$b_x$} (B);
        \draw (w) --node[inner sep=0pt, fill=white, outer sep=1pt] {$d_x$} (D);
        \draw (w) --node[inner sep=0pt, fill=white, outer sep=1pt] {$u_x$} (Un);
        
        % Punkt bei opinion machen
        \shadedraw[ball color=grey] (w) circle (0.5pt);
        
    \end{tikzpicture}
%\end{document}
